FOOD: Fast Out-Of-Distribution Detector

Deep neural networks (DNNs) perform well at classifying inputs associated with the classes they have been trained on, which are known as in distribution inputs. However, out-of-distribution (OOD) inputs pose a great challenge to DNNs and consequently represent a major risk when DNNs are implemented in safety-critical systems. Extensive research has been performed in the domain of OOD detection. However, current state-of-the-art methods for OOD detection suffer from at least one of the following limitations: (1) increased inference time - this limits existing methods' applicability to many real-world applications, and (2) the need for OOD training data - such data can be difficult to acquire and may not be representative enough, thus limiting the ability of the OOD detector to generalize. In this paper, we propose FOOD -- Fast Out-Of-Distribution detector -- an extended DNN classifier capable of efficiently detecting OOD samples with minimal inference time overhead. Our architecture features a DNN with a final Gaussian layer combined with the log likelihood ratio statistical test and an additional output neuron for OOD detection. Instead of using real OOD data, we use a novel method to craft artificial OOD samples from in-distribution data, which are used to train our OOD detector neuron. We evaluate FOOD's detection performance on the SVHN, CIFAR-10, and CIFAR-100 datasets. Our results demonstrate that in addition to achieving state-of-the-art performance, FOOD is fast and applicable to real-world applications.

==> tables/llr_vs_msp.tex <==
\begin{table}[b]
\caption{\mathcal{LLR} vs MSP comparison on ResNet34}
\centering
\begin{tabular}{lccc}
\hline
\multirow{$D_{in}$}     & \multirow{$D_{out}$}                                                          & \textbf{TNR95}                                                                                 & \multicolumn{1}{l}{\textbf{AUROC}}                                                             \\ \cline{3-4} 
                              &                                                                                     & \multicolumn{2}{c}{MSP /  LLR}                                                                                                                                                                  \\ \hline
\multicolumn{1}{c}{CIFAR-100} & \begin{tabular}[c]{@{}c@{}}SVHN\\ LSUN(r)\\ Tiny-Imagenet(r)\\ Isun(r)\end{tabular} & \begin{tabular}[c]{@{}c@{}}19.5 / 56.7 \\ 27.8 / 34.7\\ 27.5 / 28.6\\ 26.0 / 29.4\end{tabular} & \begin{tabular}[c]{@{}c@{}}79.3 / 92.0\\ 81.1 / 85.9\\ 80.6 /  82.5\\ 80.4 / 83.9\end{tabular} \\ \hline
\multicolumn{1}{c}{CIFAR-10}  & \begin{tabular}[c]{@{}c@{}}SVHN\\ LSUN(r)\\ Tiny-Imagenet(r)\\ Isun(r)\end{tabular} & \begin{tabular}[c]{@{}c@{}}56.2 / 93.1\\ 59.1 / 94.2\\ 51.4 / 89.2\\ 57.3 / 94.1\end{tabular}  & \begin{tabular}[c]{@{}c@{}}93.6 / 98.5\\ 93.6 / 98.7\\ 91.4 / 97.9\\ 93.0 / 98.7\end{tabular}  \\ \hline
\end{tabular}
\label{table:llr_vs_msp}
\end{table}
